Hug Reports: Supporting Expression of Appreciation between Users and Contributors of Open Source Software Packages

Contributors to open source software packages often describe feeling discouraged by the lack of positive feedback from users. This paper describes a technology probe, Hug Reports, that provides users a communication affordance within their code editors, through which users can convey appreciation to contributors of packages they use. In our field study, 18 users interacted with the probe for 3 weeks, resulting in messages of appreciation to 550 contributors, 26 of whom participated in subsequent research. Our findings show how locating a communication affordance within the code editor, and allowing users to express appreciation in terms of the abstractions they are exposed to (packages, modules, functions), can support exchanges of appreciation that are meaningful to users and contributors. Findings also revealed the moments in which users expressed appreciation, the two meanings that appreciation took on -- as a measure of utility and as an act of expressive communication -- and how contributors' reactions to appreciation were influenced by their perceived level of contribution. Based on these findings, we discuss opportunities and challenges for designing appreciation systems for open source in particular, and peer production communities more generally.

==> sections/sections-old/related.tex <==
In this section, we first describe how open source software packages are developed and distributed, with a focus on the sociotechnical infrastructures involved. Then, we describe how current practices of software consumption can present barriers to expressing appreciation. We then discuss existing systems for conveying appreciation, that our work draws on. Finally, we discuss observations from prior work that guided our attempt to design for meaningful appreciation.
\subsection{Sociotechnical organization of open source software packages}
In this work, we focus on open source software projects that are hosted on GitHub\footnote{https://github.com/}, and that are made available to users as packages. Here, we briefly describe how these projects are hosted, developed, and distributed. 

Open source software projects produce software that is licensed as ‘open source’, granting future users the rights to use it, study its source code, modify it, and redistribute it, all at no cost~\cite{hippel2003open}. The free distribution and open development practices enable, and often result in, collaborative and social practices of developing and maintaining the software, attracting contributions from distributed developers, many of whom are volunteers~\cite{krishnamurthy2006intrinsic, hippel2003open, benkler2017peer}. For this reason, open source projects have been described as instances of ``peer production''~\cite{benkler2017peer}. Today several open source software projects have become essential digital infrastructure that individual developers as well as commercial firms rely on~\cite{eghbal2016roads, benkler2017peer, geiger2021labor}. Despite growing commercialization and paid development work in open source projects~\cite{germonprez2018eight}, many projects continue to rely heavily on volunteers~\cite{zlotnick_2017_806811, eghbal2020working, champion2021underproduction}.  

With its collaborative and social practices, contemporary open source software development occurs primarily through social coding platforms~\cite{dabbish2012social, dabbish2012leveraging}, most notably GitHub. Social coding platforms provide code hosting capabilities and social features that support collaboration~\cite{dabbish2012social}. This includes features that increase visibility into development activity~\cite{dabbish2012leveraging} as well as channels for communication~\cite{dabbish2012social}. On GitHub, which is the most popular social coding platform~\cite{hsieh2023nip, li2021code}, projects are organized as repositories; a project’s \textbf{repository} contains its source code and hosts the conversations surrounding the project. Permissions to make \textbf{commits} (applying a code patch) to the hosted version of the source code are restricted to those designated as owners or collaborators on the repository. Developers who do not have such permissions, can nonetheless author code patches and work with owners or collaborators who can apply the patches on their behalf. In this work, we use the term `contributor' to mean any developer who has authored a code patch that has eventually been applied to the hosted version, and the term `maintainer' to refer to the subset of contributors who have commit permissions. Any developer interested in keeping track of a project, can \textbf{star} the repository. In each repository, developers who are contributors or users can track ideas, feedback, tasks, and bugs by creating \textbf{issues}. When a developer hopes to contribute a code patch to the project, they can open a \textbf{pull request}, a special issue that hosts conversations concerning the contribution. Activities on GitHub leave public traces. This provides visibility into software development activities at the level of actions provided by GitHub, and the underlying Git version control system~\cite{dabbish2012social}.

While development activities take place on GitHub, use often occurs elsewhere. Many projects are part of a larger ``software ecosystem''~\cite{bogart2021and, valiev2018ecosystem}, which Bogart et al. define as ``communities built around
shared programming languages, shared platforms, or shared dependency management tools, allowing developers to create packages that import and build on each others’ functionality''~\cite{bogart2021and}. Within an ecosystem (e.g. npm which is the JavaScript ecosystem or PyPI which is the Python ecosystem), each project is packaged for use, indexed and advertised in a registry, and made available for installation via a package manager~\cite{bogart2021and}, which a user can access through a terminal in their development environment. It is through this distribution channel~\cite{mancinelli2006managing} that many projects are consumed, often from within a development environment.  


\subsection{Barriers to expressing appreciation in open source}
Within developer communities~\cite{Mayes, Hammer_2021, Lawson_2017} as well as academic literature~\cite{raman2020stress, miller2022did, hsieh2023nip}, there is growing recognition of how working in open source projects can often feel demotivating and stressful. Open source practitioners have shared experiences~\cite{Hammer_2021, Lawson_2017} about how their interactions with users can feel like a ``constant stream of negativity''~\cite{Lawson_2017}. One reason why interactions can feel overwhelmingly negative is that contributors rarely receive positive feedback and appreciation from the users who benefit from their, often voluntary, labor. Nic Crane, a maintainer of Apache Arrow, suggests: ``we have lots of happy but quiet users''~\cite{Mayes}. With little appreciation, contributors are left facing a stream of user demands and requests, some of which are even aggressive in their tone~\cite{raman2020stress, miller2022did}. In many discussions, the lack of positive feedback and recognition are often discussed as a cause of demotivation and burnout~\cite{Mayes, hsieh2023nip, raman2020stress}.

Based on the sociotechnical organization of open source packages, we suggest three intersecting reasons why users of open source software packages rarely express appreciation to contributors. We do not intend to suggest this is a complete or comprehensive list of all contributing factors, however, we believe these observations provide a valuable starting point for positive intervention:

\subsubsection{Existing communication channels de-emphasize appreciation} Even though GitHub provides channels through which users can interact with contributors of a project, these channels were designed with values of efficiency and productivity in mind. GitHub ``Issues''\footnote{https://docs.github.com/en/issues/tracking-your-work-with-issues/about-issues}, for instance, are advertised as a way to ``track ideas, feedback, tasks, or bugs for work on GitHub''. To support effective tracking of tasks, projects can further customize the feature to provide users default issue templates for common communication such as bug reporting or feature requests\footnote{https://docs.github.com/en/communities/using-templates-to-encourage-useful-issues-and-pull-requests/configuring-issue-templates-for-your-repository}. Together, the name, advertised purpose, and user defaults normatively discourage appreciation. With hesitation, motivated users still reappropriate GitHub's features to convey appreciation, as visible in issue \#2264 in the react boilerplate project\footnote{https://github.com/react-boilerplate/react-boilerplate/issues/2264}, which is titled: ``I don't know how to thank, and show my appreciation, to the contributors on a good way''. GitHub users have pointed out how the reaction palette available within issues and pull requests lacks emojis to convey the sentiment of ``Thank you''\footnote{https://github.com/orgs/community/discussions/38201}. While stars can be used to convey appreciation, they are also intended to function as a bookmarking tool, and a way for the platform to learn user preferences\footnote{https://docs.github.com/en/get-started/exploring-projects-on-github/saving-repositories-with-stars}, which obscures the intention behind `starring'. 

\subsubsection{Establishing contact with contributors requires effort} Channels for communicating with contributors, like GitHub and email, are separate from the code editors where packages are used. To contact contributors, users need to find the right GitHub repository and then either open an issue or locate the contributor's contact details. Users are more likely to undertake this effort to report issues, since improvements can directly benefit them, than to express appreciation, from which they might not see any direct benefits. This tendency for negative feedback over positive is also observed in consumer research, showing that customers with bad experiences are more inclined to leave online reviews than those with good experiences~\cite{han2020customer, anderson1998customer}.  

\subsubsection{Packaging detaches the software from the contributors, de-emphasizing the social nature of the exchange} In his book ``Exchange and Power in Social Life''~\cite{blau2017exchange}, Blau argues that ``only social exchange tends to engender feelings of personal obligation, gratitude, and trust; purely economic exchange as such does not.'' We suggest, the current practice of distributing and consuming software as packages, reinscribes a view of software as an economic commodity~\cite{widder2023dislocated} rather than a gift of labor~\cite{Hammer_2021, terranova2000free}. By making the labor of contributors invisible, packaging de-emphasizes the social nature of the exchange and can diminish feelings of gratitude towards the contributors.   

\subsection{Appreciation systems in peer production}
Our work draws on other systems that attempt to mediate exchanges of appreciation.  Following Spiro et al.~\cite{spiro2016networks}, we use the term ``appreciation systems'' to refer to platforms through which users exchange thanks and praise. In describing related efforts, we consider different forms of exchange---whether or monetary or non-monetary---as ``appreciation'' if they involve \textit{unspecified} obligations~\cite{blau2017exchange}. For example, we are not contractually required to send messages of appreciation, make donations, or tip; we do so spontaneously. Unlike a formal trade or contract, the exact nature of the exchange is not stipulated in advance~\cite{blau2017exchange, smith2010theory}. In their work, Spiro et al. analyze several appreciation systems designed for the workplace, outlining the various dimensions along which they differed. Some of these dimensions were: (1) the \textit{audience} to whom the exchanges were visible; (2) whether the exchanges were associated with \textit{rewards} in the form of bonuses; and (3) whether they provided aggregated \textit{reporting and analytics}. Although their analysis focused on workplaces, where appreciation systems are often introduced to support appraisal in addition to gratitude~\cite{spiro2016networks}, we believe the dimensions they describe in their work outline a design space for appreciation systems, more generally. Through the process of designing our prototype, we describe the decisions we made along these dimensions.

Prior work has studied several systems through which users of open source software can \textit{reward} specific contributors individually~\cite{overney2020not, zhang2022and}\footnote{We do not consider ``bounties'' as appreciation since they are similar to contracts in that they stipulate the exact nature of the exchange.}. This includes systems such as PayPal and Patreon which contributors may link to from their personal websites. Similarly, GitHub has the `Sponsors' feature through which users of the platform can sponsor individual developers. Other platforms such as OpenCollective allow projects as a whole to accept monetary donations from users. Our work complements these systems, supporting forms of appreciation that do not involve monetary rewards but that may nonetheless improve the experiences of contributors working on open source projects. 


In the process of our research, we came across two systems, developed by open source contributors, with similar goals. The `Say Thanks'\footnote{https://github.com/BlitzKraft/saythanks.io} project provides a link that contributors can include to the repository of a project, and that users can visit to send messages of appreciation. In contrast, our work explores a communication affordance within the user's development environment recognizing how users install and use many open source packages without ever visiting the corresponding repository. The second project, called `appreciate'\footnote{https://github.com/musically-ut/appreciate}, reappropriates stars as a way to convey appreciation. It indicates to users which installed packages they have and haven't starred, from within their terminal. However, to then star the project, users still have to visit the repository. Further, we are not aware of any formal field validations of these systems. Our work builds on these efforts while also attempting to validate our approach in the field. Most directly related to our work, is Wikipedia's ``Thanks'' system~\cite{matiasdiffusion, goel2019thanks}, through which editors can thank each other. A "thank" link is shown next to each edit in the history view of an article. Clicking the link triggers a notification to the author of the edit, which includes the name of the person who thanked them. We drew on the idea of having a communication affordance located where users ultimately consume the product of contributors' efforts. 
\ed{
\subsection{Tradeoffs between }
To counter the above barriers and encourage appreciation, we were interested in lowering the effort required, and to remind users of the contributors behind the packages they rely on. At the same time we wanted the exchanges of appreciation to be meaningful to the people involved. While low effort actions can encourage interactions, prior work suggests these interactions can feel limited in the authenticity~\cite{monroy2011computers, zhang2022auggie} and support~\cite{wohn2016affective} they convey. We draw on two observations from prior work, in designing for meaningful appreciation:

\subsubsection{Procedural effort is valued less than personal effort} In the context of interpersonal communication, Markopoulos distinguishes between \textit{procedural effort}, which he describes as ``the effort that one needs to expend in order to operate a system''~\cite{markopoulos2009design}  (examples in our context would include logging in, navigating to a repository, opening an issue) and \textit{personal effort}, which he describes as ``the effort put to attend personally to an individual''~\cite{markopoulos2009design} (which in our context would be composing a message to the contributor). Prior work suggests procedural effort tends not to be valued~\cite{markopoulos2009design, zhang2022auggie} and that it can be minimized to create greater opportunities for personal effort, which is what makes the communication feel special to recipients~\cite{romero2007connecting, markopoulos2009design}. Thus, in our work, we specifically focus on lowering \textit{procedural effort} in expressing appreciation to make appreciation more approachable.

\subsubsection{"Action can be coerced, but coerced show of feeling is only a show.” (Erving Goffman, Asylums~\cite{goffman1961asylums})} Scholars studying social exchange have often noted how the introduction of social rewards or sanctions to encourage actions of reciprocity can rob those actions of their significance~\cite{blau2017exchange, goffman1961asylums}. Insofar as appreciation is a voluntary reciprocal exchange~\cite{simmel1950sociology, smith2010theory}, encouraging appreciation by introducing psychological reward mechanisms for users could diminish the meaning of the exchange for both users and contributors. So, we wanted to design a system that would subtly remind users to appreciate contributors but would not feel coercive.
}
